HoughCL: Finding Better Positive Pairs in Dense Self-supervised Learning

Recently, self-supervised methods show remarkable achievements in image-level representation learning. Nevertheless, their image-level self-supervisions lead the learned representation to sub-optimal for dense prediction tasks, such as object detection, instance segmentation, etc. To tackle this issue, several recent self-supervised learning methods have extended image-level single embedding to pixel-level dense embeddings. Unlike image-level representation learning, due to the spatial deformation of augmentation, it is difficult to sample pixel-level positive pairs. Previous studies have sampled pixel-level positive pairs using the winner-takes-all among similarity or thresholding warped distance between dense embeddings. However, these naive methods can be struggled by background clutter and outliers problems. In this paper, we introduce Hough Contrastive Learning (HoughCL), a Hough space based method that enforces geometric consistency between two dense features. HoughCL achieves robustness against background clutter and outliers. Furthermore, compared to baseline, our dense positive pairing method has no additional learnable parameters and has a small extra computation cost. Compared to previous works, our method shows better or comparable performance on dense prediction fine-tuning tasks.

==> figures/accfluc.tex <==
\begin{figure}[t]
\captionsetup[subfigure]{aboveskip=1pt,belowskip=-1pt}
\centering
\begin{subfigure}{0.49\columnwidth}
    \includegraphics[width=\textwidth]{figures/accfluc/acc_fluc_TE0.pdf}
    \caption{\textit{Art painting}}
\end{subfigure}
\begin{subfigure}{0.49\columnwidth}
    \includegraphics[width=\textwidth]{figures/accfluc/acc_fluc_TE1.pdf}
    \caption{\textit{Cartoon}}
\end{subfigure}
\\ 
\begin{subfigure}{0.49\columnwidth}
    \includegraphics[width=\textwidth]{figures/accfluc/acc_fluc_TE2.pdf}
    \caption{\textit{Photo}}
\end{subfigure}
\begin{subfigure}{0.49\columnwidth}
    \includegraphics[width=\textwidth]{figures/accfluc/acc_fluc_TE3.pdf}
    \caption{\textit{Sketch}}
\end{subfigure}
\\ 
\begin{subfigure}{0.8\columnwidth}
    \includegraphics[width=\textwidth]{figures/accfluc/acc_fluc_legend.pdf}
\end{subfigure}

\caption{\textbf{Validation accuracies for in-domains.} The X and Y-axis indicate the number of iterations and accuracy, respectively, about the validation domains (legend) and the test domain (caption). The vertical dot lines represent the starting and end points of the stochastic weights combined by SWA. 
%See the Section~\ref{s__connection_to_swa} for more details.
}% X-axis indicates the number of iterations and y-axis indicates accuracy. Captions indicate target domains and line plots show accuracies of validation domains. The vertical dot lines represent the starting and end points of the stochastic weights combined by SWA.}
\label{fig:accfluc}
\vspace{-0.7em}
\end{figure}

==> figures/additional_loss_spaces.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Loss Surfaces for \data{PACS}}
\begin{figure}[H]
\centering
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE0_env1_in_loss_plane.pdf}
    \caption{\textit{Cartoon} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE0_env2_in_loss_plane.pdf}
    \caption{\textit{Photo} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE0_env3_in_loss_plane.pdf}
    \caption{\textit{Sketch} \scriptsize{(train)}}
\end{subfigure}
\\
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE0_env1_out_loss_plane.pdf}
    \caption{\textit{Cartoon} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE0_env2_out_loss_plane.pdf}
    \caption{\textit{Photo} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE0_env3_out_loss_plane.pdf}
    \caption{\textit{Sketch} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE0_env0_in_loss_plane.pdf}
    \caption{\textit{Art painting} \scriptsize{(test)}}
\end{subfigure}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for \data{PACS} when the target domain is \textit{Art painting}.}
}
\label{figure:add_loss_surface_PACS_Art painting}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
\centering
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE1_env0_in_loss_plane.pdf}
    \caption{\textit{Art painting} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE1_env2_in_loss_plane.pdf}
    \caption{\textit{Photo} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE1_env3_in_loss_plane.pdf}
    \caption{\textit{Sketch} \scriptsize{(train)}}
\end{subfigure}
\\
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE1_env0_out_loss_plane.pdf}
    \caption{\textit{Art painting} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE1_env2_out_loss_plane.pdf}
    \caption{\textit{Photo} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE1_env3_out_loss_plane.pdf}
    \caption{\textit{Sketch} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE1_env1_in_loss_plane.pdf}
    \caption{\textit{Cartoon} \scriptsize{(test)}}
\end{subfigure}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for \data{PACS} when the target domain is \textit{Cartoon}.}
}
\label{figure:add_loss_surface_PACS_Cartoon}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
\centering
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE2_env0_in_loss_plane.pdf}
    \caption{\textit{Art painting} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE2_env1_in_loss_plane.pdf}
    \caption{\textit{Cartoon} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE2_env3_in_loss_plane.pdf}
    \caption{\textit{Sketch} \scriptsize{(train)}}
\end{subfigure}
\\
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE2_env0_out_loss_plane.pdf}
    \caption{\textit{Art painting} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE2_env1_out_loss_plane.pdf}
    \caption{\textit{Cartoon} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE2_env3_out_loss_plane.pdf}
    \caption{\textit{Sketch} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE2_env2_in_loss_plane.pdf}
    \caption{\textit{Photo} \scriptsize{(test)}}
\end{subfigure}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for \data{PACS} when the target domain is \textit{Photo}.}
}
\label{figure:add_loss_surface_PACS_Photo}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
\centering
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE3_env0_in_loss_plane.pdf}
    \caption{\textit{Art painting} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE3_env1_in_loss_plane.pdf}
    \caption{\textit{Cartoon} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE3_env2_in_loss_plane.pdf}
    \caption{\textit{Photo} \scriptsize{(train)}}
\end{subfigure}
\\
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE3_env0_out_loss_plane.pdf}
    \caption{\textit{Art painting} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE3_env1_out_loss_plane.pdf}
    \caption{\textit{Cartoon} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE3_env2_out_loss_plane.pdf}
    \caption{\textit{Photo} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/PACS/TE3_env3_in_loss_plane.pdf}
    \caption{\textit{Sketch} \scriptsize{(test)}}
\end{subfigure}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for \data{PACS} when the target domain is \textit{Sketch}.}
}
\label{figure:add_loss_surface_PACS_Sketch}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Loss Surfaces for \data{VLCS}}
\begin{figure}[H]
\centering
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE0_env1_in_loss_plane.pdf}
    \caption{\textit{LabelMe} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE0_env2_in_loss_plane.pdf}
    \caption{\textit{SUN09} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE0_env3_in_loss_plane.pdf}
    \caption{\textit{VOC2007} \scriptsize{(train)}}
\end{subfigure}
\\
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE0_env1_out_loss_plane.pdf}
    \caption{\textit{LabelMe} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE0_env2_out_loss_plane.pdf}
    \caption{\textit{SUN09} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE0_env3_out_loss_plane.pdf}
    \caption{\textit{VOC2007} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE0_env0_in_loss_plane.pdf}
    \caption{\textit{Caltech101} \scriptsize{(test)}}
\end{subfigure}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for \data{VLCS} when the target domain is \textit{Caltech101}.}
}
\label{figure:add_loss_surface_VLCS_Caltech101}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
\centering
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE1_env0_in_loss_plane.pdf}
    \caption{\textit{Caltech101} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE1_env2_in_loss_plane.pdf}
    \caption{\textit{SUN09} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE1_env3_in_loss_plane.pdf}
    \caption{\textit{VOC2007} \scriptsize{(train)}}
\end{subfigure}
\\
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE1_env0_out_loss_plane.pdf}
    \caption{\textit{Caltech101} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE1_env2_out_loss_plane.pdf}
    \caption{\textit{SUN09} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE1_env3_out_loss_plane.pdf}
    \caption{\textit{VOC2007} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE1_env1_in_loss_plane.pdf}
    \caption{\textit{LabelMe} \scriptsize{(test)}}
\end{subfigure}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for \data{VLCS} when the target domain is \textit{LabelMe}.}
}
\label{figure:add_loss_surface_VLCS_LabelMe}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
\centering
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE2_env0_in_loss_plane.pdf}
    \caption{\textit{Caltech101} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE2_env1_in_loss_plane.pdf}
    \caption{\textit{LabelMe} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE2_env3_in_loss_plane.pdf}
    \caption{\textit{VOC2007} \scriptsize{(train)}}
\end{subfigure}
\\
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE2_env0_out_loss_plane.pdf}
    \caption{\textit{Caltech101} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE2_env1_out_loss_plane.pdf}
    \caption{\textit{LabelMe} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE2_env3_out_loss_plane.pdf}
    \caption{\textit{VOC2007} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE2_env2_in_loss_plane.pdf}
    \caption{\textit{SUN09} \scriptsize{(test)}}
\end{subfigure}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for \data{VLCS} when the target domain is \textit{SUN09}.}
}
\label{figure:add_loss_surface_VLCS_SUN09}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
\centering
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE3_env0_in_loss_plane.pdf}
    \caption{\textit{Caltech101} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE3_env1_in_loss_plane.pdf}
    \caption{\textit{LabelMe} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE3_env2_in_loss_plane.pdf}
    \caption{\textit{SUN09} \scriptsize{(train)}}
\end{subfigure}
\\
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE3_env0_out_loss_plane.pdf}
    \caption{\textit{Caltech101} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE3_env1_out_loss_plane.pdf}
    \caption{\textit{LabelMe} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE3_env2_out_loss_plane.pdf}
    \caption{\textit{SUN09} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/VLCS/TE3_env3_in_loss_plane.pdf}
    \caption{\textit{VOC2007} \scriptsize{(test)}}
\end{subfigure}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for \data{VLCS} when the target domain is \textit{VOC2007}.}
}
\label{figure:add_loss_surface_VLCS_VOC2007}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Loss Surfaces for \data{OfficeHome}}
\begin{figure}[H]
\centering
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE0_env1_in_loss_plane.pdf}
    \caption{\textit{Clipart} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE0_env2_in_loss_plane.pdf}
    \caption{\textit{Product} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE0_env3_in_loss_plane.pdf}
    \caption{\textit{Real world} \scriptsize{(train)}}
\end{subfigure}
\\
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE0_env1_out_loss_plane.pdf}
    \caption{\textit{Clipart} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE0_env2_out_loss_plane.pdf}
    \caption{\textit{Product} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE0_env3_out_loss_plane.pdf}
    \caption{\textit{Real world} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE0_env0_in_loss_plane.pdf}
    \caption{\textit{Art} \scriptsize{(test)}}
\end{subfigure}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for \data{OfficeHome} when the target domain is \textit{Art}.}
}
\label{figure:add_loss_surface_OfficeHome_Art}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
\centering
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE1_env0_in_loss_plane.pdf}
    \caption{\textit{Art} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE1_env2_in_loss_plane.pdf}
    \caption{\textit{Product} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE1_env3_in_loss_plane.pdf}
    \caption{\textit{Real world} \scriptsize{(train)}}
\end{subfigure}
\\
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE1_env0_out_loss_plane.pdf}
    \caption{\textit{Art} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE1_env2_out_loss_plane.pdf}
    \caption{\textit{Product} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE1_env3_out_loss_plane.pdf}
    \caption{\textit{Real world} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE1_env1_in_loss_plane.pdf}
    \caption{\textit{Clipart} \scriptsize{(test)}}
\end{subfigure}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for \data{OfficeHome} when the target domain is \textit{Clipart}.}
}
\label{figure:add_loss_surface_OfficeHome_Clipart}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
\centering
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE2_env0_in_loss_plane.pdf}
    \caption{\textit{Art} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE2_env1_in_loss_plane.pdf}
    \caption{\textit{Clipart} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE2_env3_in_loss_plane.pdf}
    \caption{\textit{Real world} \scriptsize{(train)}}
\end{subfigure}
\\
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE2_env0_out_loss_plane.pdf}
    \caption{\textit{Art} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE2_env1_out_loss_plane.pdf}
    \caption{\textit{Clipart} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE2_env3_out_loss_plane.pdf}
    \caption{\textit{Real world} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE2_env2_in_loss_plane.pdf}
    \caption{\textit{Product} \scriptsize{(test)}}
\end{subfigure}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for \data{OfficeHome} when the target domain is \textit{Product}.}
}
\label{figure:add_loss_surface_OfficeHome_Product}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
\centering
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE3_env0_in_loss_plane.pdf}
    \caption{\textit{Art} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE3_env1_in_loss_plane.pdf}
    \caption{\textit{Clipart} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE3_env2_in_loss_plane.pdf}
    \caption{\textit{Product} \scriptsize{(train)}}
\end{subfigure}
\\
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE3_env0_out_loss_plane.pdf}
    \caption{\textit{Art} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE3_env1_out_loss_plane.pdf}
    \caption{\textit{Clipart} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE3_env2_out_loss_plane.pdf}
    \caption{\textit{Product} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/OfficeHome/TE3_env3_in_loss_plane.pdf}
    \caption{\textit{Real world} \scriptsize{(test)}}
\end{subfigure}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for \data{OfficeHome} when the target domain is \textit{Real world}.}
}
\label{figure:add_loss_surface_OfficeHome_Real world}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Loss Surfaces for \data{TerraIncognita}}
\begin{figure}[H]
\centering
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE0_env1_in_loss_plane.pdf}
    \caption{\textit{Location38} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE0_env2_in_loss_plane.pdf}
    \caption{\textit{Location43} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE0_env3_in_loss_plane.pdf}
    \caption{\textit{Location46} \scriptsize{(train)}}
\end{subfigure}
\\
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE0_env1_out_loss_plane.pdf}
    \caption{\textit{Location38} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE0_env2_out_loss_plane.pdf}
    \caption{\textit{Location43} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE0_env3_out_loss_plane.pdf}
    \caption{\textit{Location46} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE0_env0_in_loss_plane.pdf}
    \caption{\textit{Location100} \scriptsize{(test)}}
\end{subfigure}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for \data{TerraIncognita} when the target domain is \textit{Location100}.}
}
\label{figure:add_loss_surface_TerraIncognita_Location100}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
\centering
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE1_env0_in_loss_plane.pdf}
    \caption{\textit{Location100} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE1_env2_in_loss_plane.pdf}
    \caption{\textit{Location43} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE1_env3_in_loss_plane.pdf}
    \caption{\textit{Location46} \scriptsize{(train)}}
\end{subfigure}
\\
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE1_env0_out_loss_plane.pdf}
    \caption{\textit{Location100} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE1_env2_out_loss_plane.pdf}
    \caption{\textit{Location43} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE1_env3_out_loss_plane.pdf}
    \caption{\textit{Location46} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE1_env1_in_loss_plane.pdf}
    \caption{\textit{Location38} \scriptsize{(test)}}
\end{subfigure}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for \data{TerraIncognita} when the target domain is \textit{Location38}.}
}
\label{figure:add_loss_surface_TerraIncognita_Location38}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
\centering
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE2_env0_in_loss_plane.pdf}
    \caption{\textit{Location100} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE2_env1_in_loss_plane.pdf}
    \caption{\textit{Location38} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE2_env3_in_loss_plane.pdf}
    \caption{\textit{Location46} \scriptsize{(train)}}
\end{subfigure}
\\
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE2_env0_out_loss_plane.pdf}
    \caption{\textit{Location100} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE2_env1_out_loss_plane.pdf}
    \caption{\textit{Location38} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE2_env3_out_loss_plane.pdf}
    \caption{\textit{Location46} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE2_env2_in_loss_plane.pdf}
    \caption{\textit{Location43} \scriptsize{(test)}}
\end{subfigure}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for \data{TerraIncognita} when the target domain is \textit{Location43}.}
}
\label{figure:add_loss_surface_TerraIncognita_Location43}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
\centering
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE3_env0_in_loss_plane.pdf}
    \caption{\textit{Location100} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE3_env1_in_loss_plane.pdf}
    \caption{\textit{Location38} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.24\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE3_env2_in_loss_plane.pdf}
    \caption{\textit{Location43} \scriptsize{(train)}}
\end{subfigure}
\\
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE3_env0_out_loss_plane.pdf}
    \caption{\textit{Location100} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE3_env1_out_loss_plane.pdf}
    \caption{\textit{Location38} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE3_env2_out_loss_plane.pdf}
    \caption{\textit{Location43} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.18\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/TerraIncognita/TE3_env3_in_loss_plane.pdf}
    \caption{\textit{Location46} \scriptsize{(test)}}
\end{subfigure}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for \data{TerraIncognita} when the target domain is \textit{Location46}.}
}
\label{figure:add_loss_surface_TerraIncognita_Location46}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Loss Surfaces for \data{DomainNet}}
\begin{figure}[H]
\centering
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE0_env1_in_loss_plane.pdf}
    \caption{\textit{Infographic} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE0_env2_in_loss_plane.pdf}
    \caption{\textit{Painting} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE0_env3_in_loss_plane.pdf}
    \caption{\textit{Quickdraw} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE0_env4_in_loss_plane.pdf}
    \caption{\textit{Real} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE0_env5_in_loss_plane.pdf}
    \caption{\textit{Sketch} \scriptsize{(train)}}
\end{subfigure}
\\
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE0_env1_out_loss_plane.pdf}
    \caption{\textit{Infographic} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE0_env2_out_loss_plane.pdf}
    \caption{\textit{Painting} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE0_env3_out_loss_plane.pdf}
    \caption{\textit{Quickdraw} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE0_env4_out_loss_plane.pdf}
    \caption{\textit{Real} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE0_env5_out_loss_plane.pdf}
    \caption{\textit{Sketch} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE0_env0_in_loss_plane.pdf}
    \caption{\textit{Clipart} \scriptsize{(test)}}
\end{subfigure}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for \data{DomainNet} when the target domain is \textit{Clipart}.}
}
\label{figure:add_loss_surface_DomainNet_Clipart}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
\centering
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE1_env0_in_loss_plane.pdf}
    \caption{\textit{Clipart} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE1_env2_in_loss_plane.pdf}
    \caption{\textit{Painting} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE1_env3_in_loss_plane.pdf}
    \caption{\textit{Quickdraw} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE1_env4_in_loss_plane.pdf}
    \caption{\textit{Real} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE1_env5_in_loss_plane.pdf}
    \caption{\textit{Sketch} \scriptsize{(train)}}
\end{subfigure}
\\
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE1_env0_out_loss_plane.pdf}
    \caption{\textit{Clipart} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE1_env2_out_loss_plane.pdf}
    \caption{\textit{Painting} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE1_env3_out_loss_plane.pdf}
    \caption{\textit{Quickdraw} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE1_env4_out_loss_plane.pdf}
    \caption{\textit{Real} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE1_env5_out_loss_plane.pdf}
    \caption{\textit{Sketch} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE1_env1_in_loss_plane.pdf}
    \caption{\textit{Infographic} \scriptsize{(test)}}
\end{subfigure}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for \data{DomainNet} when the target domain is \textit{Infographic}.}
}
\label{figure:add_loss_surface_DomainNet_Infographic}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
\centering
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE2_env0_in_loss_plane.pdf}
    \caption{\textit{Clipart} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE2_env1_in_loss_plane.pdf}
    \caption{\textit{Infographic} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE2_env3_in_loss_plane.pdf}
    \caption{\textit{Quickdraw} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE2_env4_in_loss_plane.pdf}
    \caption{\textit{Real} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE2_env5_in_loss_plane.pdf}
    \caption{\textit{Sketch} \scriptsize{(train)}}
\end{subfigure}
\\
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE2_env0_out_loss_plane.pdf}
    \caption{\textit{Clipart} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE2_env1_out_loss_plane.pdf}
    \caption{\textit{Infographic} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE2_env3_out_loss_plane.pdf}
    \caption{\textit{Quickdraw} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE2_env4_out_loss_plane.pdf}
    \caption{\textit{Real} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE2_env5_out_loss_plane.pdf}
    \caption{\textit{Sketch} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE2_env2_in_loss_plane.pdf}
    \caption{\textit{Painting} \scriptsize{(test)}}
\end{subfigure}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for \data{DomainNet} when the target domain is \textit{Painting}.}
}
\label{figure:add_loss_surface_DomainNet_Painting}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
\centering
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE3_env0_in_loss_plane.pdf}
    \caption{\textit{Clipart} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE3_env1_in_loss_plane.pdf}
    \caption{\textit{Infographic} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE3_env2_in_loss_plane.pdf}
    \caption{\textit{Painting} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE3_env4_in_loss_plane.pdf}
    \caption{\textit{Real} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE3_env5_in_loss_plane.pdf}
    \caption{\textit{Sketch} \scriptsize{(train)}}
\end{subfigure}
\\
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE3_env0_out_loss_plane.pdf}
    \caption{\textit{Clipart} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE3_env1_out_loss_plane.pdf}
    \caption{\textit{Infographic} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE3_env2_out_loss_plane.pdf}
    \caption{\textit{Painting} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE3_env4_out_loss_plane.pdf}
    \caption{\textit{Real} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE3_env5_out_loss_plane.pdf}
    \caption{\textit{Sketch} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE3_env3_in_loss_plane.pdf}
    \caption{\textit{Quickdraw} \scriptsize{(test)}}
\end{subfigure}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for \data{DomainNet} when the target domain is \textit{Quickdraw}.}
}
\label{figure:add_loss_surface_DomainNet_Quickdraw}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
\centering
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE4_env0_in_loss_plane.pdf}
    \caption{\textit{Clipart} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE4_env1_in_loss_plane.pdf}
    \caption{\textit{Infographic} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE4_env2_in_loss_plane.pdf}
    \caption{\textit{Painting} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE4_env3_in_loss_plane.pdf}
    \caption{\textit{Quickdraw} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE4_env5_in_loss_plane.pdf}
    \caption{\textit{Sketch} \scriptsize{(train)}}
\end{subfigure}
\\
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE4_env0_out_loss_plane.pdf}
    \caption{\textit{Clipart} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE4_env1_out_loss_plane.pdf}
    \caption{\textit{Infographic} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE4_env2_out_loss_plane.pdf}
    \caption{\textit{Painting} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE4_env3_out_loss_plane.pdf}
    \caption{\textit{Quickdraw} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE4_env5_out_loss_plane.pdf}
    \caption{\textit{Sketch} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE4_env4_in_loss_plane.pdf}
    \caption{\textit{Real} \scriptsize{(test)}}
\end{subfigure}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for \data{DomainNet} when the target domain is \textit{Real}.}
}
\label{figure:add_loss_surface_DomainNet_Real}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
\centering
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE5_env0_in_loss_plane.pdf}
    \caption{\textit{Clipart} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE5_env1_in_loss_plane.pdf}
    \caption{\textit{Infographic} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE5_env2_in_loss_plane.pdf}
    \caption{\textit{Painting} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE5_env3_in_loss_plane.pdf}
    \caption{\textit{Quickdraw} \scriptsize{(train)}}
\end{subfigure}
\begin{subfigure}[b]{0.19\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE5_env4_in_loss_plane.pdf}
    \caption{\textit{Real} \scriptsize{(train)}}
\end{subfigure}
\\
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE5_env0_out_loss_plane.pdf}
    \caption{\textit{Clipart} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE5_env1_out_loss_plane.pdf}
    \caption{\textit{Infographic} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE5_env2_out_loss_plane.pdf}
    \caption{\textit{Painting} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE5_env3_out_loss_plane.pdf}
    \caption{\textit{Quickdraw} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE5_env4_out_loss_plane.pdf}
    \caption{\textit{Real} \scriptsize{(valid)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\columnwidth}
    \includegraphics[width=\textwidth]{figures/all_loss_surfaces/DomainNet/TE5_env5_in_loss_plane.pdf}
    \caption{\textit{Sketch} \scriptsize{(test)}}
\end{subfigure}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for \data{DomainNet} when the target domain is \textit{Sketch}.}
}
\label{figure:add_loss_surface_DomainNet_Sketch}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> figures/depreacated_loss_space_out.tex <==
% % vertically centering
% \begin{figure*}[t]
% \centering

% \begin{subfigure}[b]{0.24\textwidth}
%     \includegraphics[width=\textwidth]{figures/loss_plane/TE2_env0_out_loss_plane.pdf}
%     \caption{\textit{Art painting}}
% \end{subfigure}
% \begin{subfigure}[b]{0.24\textwidth}
%     \includegraphics[width=\textwidth]{figures/loss_plane/TE2_env1_out_loss_plane.pdf}
%     \caption{\textit{Cartoon}}
% \end{subfigure}
% \begin{subfigure}[b]{0.24\textwidth}
%     \includegraphics[width=\textwidth]{figures/loss_plane/TE2_env3_out_loss_plane.pdf}
%     \caption{\textit{Sketch}}
% \end{subfigure}
% \begin{subfigure}[b]{0.24\textwidth}
%     \includegraphics[width=\textwidth]{figures/loss_plane/TE2_env2_in_loss_plane.pdf}
%     \caption{\textit{Photo} (test)}
% \end{subfigure}

% \caption{\textbf{Visualization Out-of-distribution loss surface when target domain is \textit{photo} in PACS dataset.} The three points such as circle, rectangle, and triangle indicate randomly chosen model weights at the end of the training phase. A plane can be defined by the three weights and losses upon the plane are visualized with certain contours.}
% \label{fig:loss_space_out}
% \end{figure*}

==> figures/deprecated_acc_fluc.tex <==
\begin{figure}[t]
\includegraphics[width=0.9\linewidth]{figures/acc_fluc_TE0.pdf}
\caption{Performance fluctuation comparison between validation and test. Standard deviations are 0.63 for validation and 3.49 for test. Art painting is used for target domain.}
\label{fig:acc_fluc}
\end{figure}

==> figures/feature_dist.tex <==
% vertically centering
\begin{figure}[t]
\begin{subfigure}{0.49\columnwidth}
    \includegraphics[width=\textwidth]{figures/feature_dist/erm_TE0.pdf}
    \caption{ERM}
\end{subfigure}
\begin{subfigure}{0.49\columnwidth}
    \includegraphics[width=\textwidth]{figures/feature_dist/dann_TE0.pdf}
    \caption{DANN}
\end{subfigure}

\caption{
%\textbf{Latent feature visualization of in-domain training examples.} t-SNE is applied to visualize the output features of the network.
\textbf{t-SNE visualization of latent features of in-domain training examples for the \data{PACS} dataset.} Each cluster implies the seven pre-defined classes. There is no significant difference between ERM and DANN, although DANN uses explicit guidance to learn domain-invariant features. Colors indicate multiple domains: \textit{cartoon}~(\textcolor{red}{red}), \textit{photo}~(\textcolor{green}{green}), and \textit{sketch}~(\textcolor{blue}{blue}) in the \data{PACS} dataset when target domain is \textit{art painting}.}
\label{fig:feature_dist}
\end{figure}

==> figures/flatness_comparison.tex <==
\begin{figure}[t]
\captionsetup[subfigure]{aboveskip=1pt,belowskip=-3pt}
\centering
\begin{subfigure}{0.49\columnwidth}
    \includegraphics[width=\textwidth]{figures/flatness/PACS_TE3_TRG3_S5_MD60_N100_BNFalse.pdf}
    \caption{\textit{Sketch} (test)}
\end{subfigure}
\begin{subfigure}{0.49\columnwidth}
    \includegraphics[width=\textwidth]{figures/flatness/PACS_TE3_TRG0_S5_MD60_N100_BNFalse.pdf}
    \caption{\textit{Art painting} (train)}
\end{subfigure}
\\ [0.5em]
\begin{subfigure}{0.49\columnwidth}
    \includegraphics[width=\textwidth]{figures/flatness/PACS_TE3_TRG1_S5_MD60_N100_BNFalse.pdf}
    \caption{\textit{Cartoon} (train)}
\end{subfigure}
\begin{subfigure}{0.49\columnwidth}
    \includegraphics[width=\textwidth]{figures/flatness/PACS_TE3_TRG2_S5_MD60_N100_BNFalse.pdf}
    \caption{\textit{Photo} (train)}
\end{subfigure}
% \\ 
% \begin{subfigure}{0.33\columnwidth}
%     \includegraphics[width=\textwidth]{figures/flatness/legend.pdf}
% \end{subfigure}

\caption{\textbf{Flatness comparison between SWA and ERM.} X-axis indicates distances from original weight and Y-axis indicates test or train error. Each error point is averaged over 100 runs and its standard deviation is shown as shaded area. The directions are randomly sampled from uniform distribution on the unit sphere.
%Details are denoted in Section~\ref{s__connection_to_swa}.
}
\label{fig:flatness}
\vspace{-0.4cm}
\end{figure}

==> figures/loss_shapes.tex <==
% \begin{figure}[t]
% \centering
% \begin{subfigure}[t]{0.24\columnwidth}
%     \includegraphics[width=\textwidth]{figures/loss_shapes/VLCS_TE0_in_loss_plane.pdf}
%     \caption{\data{VL} (train)}
% \end{subfigure}
% \begin{subfigure}[t]{0.24\columnwidth}
%     \includegraphics[width=\textwidth]{figures/loss_shapes/OH_TE0_in_loss_plane.pdf}
%     \caption{\data{OH} (train)}
% \end{subfigure}
% \begin{subfigure}[t]{0.24\columnwidth}
%     \includegraphics[width=\textwidth]{figures/loss_shapes/TR_TE0_in_loss_plane.pdf}
%     \caption{\data{TI} (train)}
% \end{subfigure}
% \begin{subfigure}[t]{0.24\columnwidth}
%     \includegraphics[width=\textwidth]{figures/loss_shapes/DN_TE0_in_loss_plane.pdf}
%     \caption{\data{DN} (train)}
% \end{subfigure}
% \\[0.5em]
% \begin{subfigure}[b]{0.24\columnwidth}
%     \includegraphics[width=\textwidth]{figures/loss_shapes/VLCS_TE0_env0_in_loss_plane.pdf}
%     \caption{\data{VL} (test)}
% \end{subfigure}
% \begin{subfigure}[b]{0.24\columnwidth}
%     \includegraphics[width=\textwidth]{figures/loss_shapes/OH_TE0_env0_in_loss_plane.pdf}
%     \caption{\data{OH} (test)}
% \end{subfigure}
% \begin{subfigure}[b]{0.24\columnwidth}
%     \includegraphics[width=\textwidth]{figures/loss_shapes/TR_TE0_env0_in_loss_plane.pdf}
%     \caption{\data{TI} (test)}
% \end{subfigure}
% \begin{subfigure}[b]{0.24\columnwidth}
%     \includegraphics[width=\textwidth]{figures/loss_shapes/DN_TE0_env0_in_loss_plane.pdf}
%     \caption{\data{DN} (test)}
% \end{subfigure}

% \caption{\textbf{Visualization of loss surfaces for various datasets.} }
% \label{fig:loss_shapes}
% \end{figure}


\begin{figure}[t]
\centering
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{0.5}
\begin{tabular}{m{0.8em}cccc}
\rotatebox[origin=c]{90}{\small{Train}} &
\makecell{\includegraphics[width=0.23\columnwidth]{figures/loss_shapes/VLCS_TE0_in_loss_plane.pdf}} &
\makecell{\includegraphics[width=0.23\columnwidth]{figures/loss_shapes/OH_TE0_in_loss_plane.pdf}} &
\makecell{\includegraphics[width=0.23\columnwidth]{figures/loss_shapes/TR_TE0_in_loss_plane.pdf}} &
\makecell{\includegraphics[width=0.23\columnwidth]{figures/loss_shapes/DN_TE0_in_loss_plane.pdf}}
\\
\rotatebox[origin=c]{90}{\small{Test}} &
\makecell{\includegraphics[width=0.23\columnwidth]{figures/loss_shapes/VLCS_TE0_env0_in_loss_plane.pdf}} &
\makecell{\includegraphics[width=0.23\columnwidth]{figures/loss_shapes/OH_TE0_env0_in_loss_plane.pdf}} &
\makecell{\includegraphics[width=0.23\columnwidth]{figures/loss_shapes/TR_TE0_env0_in_loss_plane.pdf}} &
\makecell{\includegraphics[width=0.23\columnwidth]{figures/loss_shapes/DN_TE0_env0_in_loss_plane.pdf}}
\\
& \data{\scriptsize{VLCS}} & \data{\scriptsize{OfficeHome}} & \data{\scriptsize{Terra}} & \data{\scriptsize{DomainNet}}
\\
& & & \data{\scriptsize{Incognita}} &
\end{tabular}
\caption{\textbf{Visualization of loss surface shapes for various datasets.} Each plane is defined by three model weights. First and second rows present shapes of averaged training loss surfaces and shapes of test loss surfaces, respectively. First domain of each dataset is used for target domain, in alphabetical order: \textit{Caltech101} for \data{VLCS}, \textit{Art} for \data{OfficeHome}, \textit{Location100} for \data{TerraIncognita}, and \textit{Clipart} for \data{DomainNet}. Most of contours follow ellipse shapes, independent to dataset. More visualizations of loss surface is given in Appendix.}
\label{fig:loss_shapes}
\end{figure}

==> figures/loss_space.tex <==
% vertically centering
\begin{figure*}[t]
\centering
%\raggedright
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{figures/loss_plane/TE2_env0_in_loss_plane.pdf}
    \caption{\textit{Art painting} (train)}
\end{subfigure}
\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{figures/loss_plane/TE2_env1_in_loss_plane.pdf}
    \caption{\textit{Cartoon} (train)}
\end{subfigure}
\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{figures/loss_plane/TE2_env3_in_loss_plane.pdf}
    \caption{\textit{Sketch} (train)}
\end{subfigure}
\\
\raggedright
\begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{figures/loss_plane/TE2_env0_out_loss_plane.pdf}
    \caption{\textit{Art painting} (valid)}
\end{subfigure}
\begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{figures/loss_plane/TE2_env1_out_loss_plane.pdf}
    \caption{\textit{Cartoon} (valid)}
\end{subfigure}
\begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{figures/loss_plane/TE2_env3_out_loss_plane.pdf}
    \caption{\textit{Sketch} (valid)}
\end{subfigure}
\begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{figures/loss_plane/TE2_env2_in_loss_plane.pdf}
    \caption{\textit{Photo} (test)}
\end{subfigure}

\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for multiple domains in \data{PACS} dataset when the target domain is \textit{photo}. 
%In-distribution loss surface when target domain is \textit{photo} in PACS dataset.
} The three points such as circle, rectangle, and triangle indicate model weights chosen at the end of training phase with equal intervals. Each plane is defined by the three weights and losses upon the plane are visualized with certain contours. The training loss surfaces (a, b, c) look similar by sharing a big valley near the three weights but the domain shifts can be observed in the loss surfaces of validation and test datasets (d, e, f, g).}
\vspace{-1.0em}
\label{fig:loss_space}
\end{figure*}

==> figures/loss_space_more.tex <==
\begin{figure}[t]
\centering
\setlength{\tabcolsep}{0.5pt}
\renewcommand{\arraystretch}{0.1}
\begin{tabular}{m{0.8em}cccc}
\rotatebox[origin=c]{90}{\small Train 1} &
\makecell{\includegraphics[width=0.22\columnwidth]{figures/loss_plane_more/VLCS_TE0_env1_in_loss_plane.pdf}} &
\makecell{\includegraphics[width=0.22\columnwidth]{figures/loss_plane_more/OH_TE0_env1_in_loss_plane.pdf}} &
\makecell{\includegraphics[width=0.22\columnwidth]{figures/loss_plane_more/TR_TE0_env1_in_loss_plane.pdf}} &
\makecell{\includegraphics[width=0.22\columnwidth]{figures/loss_plane_more/DN_TE0_env1_in_loss_plane.pdf}}
\\
\rotatebox[origin=c]{90}{\small{Train 2}} &
\makecell{\includegraphics[width=0.22\columnwidth]{figures/loss_plane_more/VLCS_TE0_env2_in_loss_plane.pdf}} &
\makecell{\includegraphics[width=0.22\columnwidth]{figures/loss_plane_more/OH_TE0_env2_in_loss_plane.pdf}} &
\makecell{\includegraphics[width=0.22\columnwidth]{figures/loss_plane_more/TR_TE0_env2_in_loss_plane.pdf}} &
\makecell{\includegraphics[width=0.22\columnwidth]{figures/loss_plane_more/DN_TE0_env2_in_loss_plane.pdf}}
\\
\rotatebox[origin=c]{90}{\small{Train 3}} &
\makecell{\includegraphics[width=0.22\columnwidth]{figures/loss_plane_more/VLCS_TE0_env3_in_loss_plane.pdf}} &
\makecell{\includegraphics[width=0.22\columnwidth]{figures/loss_plane_more/OH_TE0_env3_in_loss_plane.pdf}} &
\makecell{\includegraphics[width=0.22\columnwidth]{figures/loss_plane_more/TR_TE0_env3_in_loss_plane.pdf}} &
\makecell{\includegraphics[width=0.22\columnwidth]{figures/loss_plane_more/DN_TE0_env3_in_loss_plane.pdf}}
\\
\rotatebox[origin=c]{90}{\small{Test}} &
\makecell{\includegraphics[width=0.22\columnwidth]{figures/loss_plane_more/VLCS_TE0_env0_in_loss_plane.pdf}} &
\makecell{\includegraphics[width=0.22\columnwidth]{figures/loss_plane_more/OH_TE0_env0_in_loss_plane.pdf}} &
\makecell{\includegraphics[width=0.22\columnwidth]{figures/loss_plane_more/TR_TE0_env0_in_loss_plane.pdf}} &
\makecell{\includegraphics[width=0.22\columnwidth]{figures/loss_plane_more/DN_TE0_env0_in_loss_plane.pdf}}
\\
& \data{\scriptsize{VLCS}} & \data{\scriptsize{OfficeHome}} & \data{\scriptsize{Terra}} & \data{\scriptsize{DomainNet}}
\\
& & & \data{\scriptsize{Incognita}} &
\end{tabular}
\vspace{-0.5em}
\caption{\textbf{Visualization of loss surfaces for various datasets.} 
%Each plane is defined by three model weights. From first to third rows present shapes of training loss surfaces for each training domains, and fourth row shows shapes of test loss surfaces. 
First domain of each dataset is used for target domain, in alphabetical order: \textit{Caltech101} for \data{VLCS}, \textit{Art} for \data{OfficeHome}, \textit{Location100} for \data{TerraIncognita}, and \textit{Clipart} for \data{DomainNet}. 
%For \data{DomainNet}, the figure only show training loss surfaces of first three domains among five.
}
\vspace{-1.0em}
\label{fig:loss_shapes}
\end{figure}
